Sample-Efficient Reinforcement Learning Is Feasible for Linearly Realizable MDPs with Limited Revisiting

Low-complexity models such as linear function representation play a pivotal role in enabling sample-efficient reinforcement learning (RL). The current paper pertains to a scenario with value-based linear representation, which postulates the linear realizability of the optimal Q-function (also called the "linear $Q^{\star}$ problem"). While linear realizability alone does not allow for sample-efficient solutions in general, the presence of a large sub-optimality gap is a potential game changer, depending on the sampling mechanism in use. Informally, sample efficiency is achievable with a large sub-optimality gap when a generative model is available but is unfortunately infeasible when we turn to standard online RL settings. In this paper, we make progress towards understanding this linear $Q^{\star}$ problem by investigating a new sampling protocol, which draws samples in an online/exploratory fashion but allows one to backtrack and revisit previous states in a controlled and infrequent manner. This protocol is more flexible than the standard online RL setting, while being practically relevant and far more restrictive than the generative model. We develop an algorithm tailored to this setting, achieving a sample complexity that scales polynomially with the feature dimension, the horizon, and the inverse sub-optimality gap, but not the size of the state/action space. Our findings underscore the fundamental interplay between sampling protocols and low-complexity structural representation in RL.

==> analysis.tex <==
\section{Analysis}

Before proceeding, we introduce several convenient notation to be used throughout the proof.
For any $(s,a,h) \in \cS\times \cA \times [H]$, we abbreviate 
%
\begin{align}
	P_{h, s,a} \defn P_h(\cdot \mymid s,a) \in \mathbb{R}^{|\cS|}. 
\end{align}
%
For any time step $h$ in the $k$-th (re)-visiting attempt,
we define the empirical distribution vector $P_h^k \in \mathbb{R}^{|\cS|}$  such that
%
\begin{align}
	P_h^k(s) \defn \begin{cases} 1, &\text{if }s = s_{h+1}^k; \\ 0,  &\text{if }s \ne s_{h+1}^k. \end{cases}
\end{align}
%
The value function estimate $V_{h}^k: \cS \rightarrow \mathbb{R}$ associated with the $k$-th (re)-visiting attempt and time step $h$ is defined as
%
\begin{align}
 \label{defn:V-Q}
	\forall (s,h,k) \in \cS \times [H] \times [K]: \qquad V_h^{k}(s) \coloneqq  \max_{a\in \cA} Q_h^{k}(s,a) ,
\end{align}
%
where the iterate $Q_h^{k}$ is defined in Algorithm~\ref{alg:linearQ}. 


To bound the regret for our proposed estimate, we first note the simple relation  
\begin{align}
\label{eqn:buenos-aires}
\sum_{k = 1}^K \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big] 
\le 
\sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big] + H\left(K-\left|\mathcal{I}_{1}^K\right|\right),
\end{align}
where we use the fact that $V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)$ is uniformly 
bounded by $H$.
It is thus sufficient to bound each term on the right hand side separately. 
For $K-\left|\mathcal{I}_{1}^K\right|$, we make the key observation that
\begin{align}
K-\left|\mathcal{I}_{1}^K\right| = \sum_{h = 1}^H\left(\left|\mathcal{I}_{h+1}^K\right|-\left|\mathcal{I}_{h}^K\right|\right) \le \frac{c^2d^2H^5\log^2 \frac{K}{\delta}}{\tau^2}. \label{eq:number-leafs}
\end{align} 
Here the last inequality comes from the following lemma, whose proof is provided in Section~\ref{sec:invierno-porteno}.
\begin{lemma}  \label{lem:number-nodes}
For any $1 \le h \le H$, with probability at least $1-\delta$,
\begin{align}
\left|\mathcal{I}_{h+1}^K \setminus \mathcal{I}_{h}^K\right| \le \frac{c^2d^2H^4\log^2 \frac{K}{\delta}}{\tau^2}. \label{eqn:restarts}
\end{align}
\end{lemma}


Now we are only left to control term $\sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big]$ in expression~\eqref{eqn:buenos-aires}.
Towards this end, let us first prove that the estimate $Q_h^k(s, a)$, delivered by Algorithm~\ref{alg:linearQ}, obeys the following result. The proof of this result is postponed to Section~\ref{sec:pf-lem-qk}. 

\begin{lemma} \label{lem:Qk-error}
With probability at least $1-\delta$, 
\begin{equation}
0 \le Q_h^k(s, a) - Q_h^{\star}(s, a) \le b_h^k(s, a), \label{eq:Qk-error}
\end{equation}
holds simultaneously for all $1 \le k \le K$ and all $(s, a) \in \cS \times \cA$.
\end{lemma}
\ytw{after applying the union bound, the log term in $b_h^k$ may change.}

To control the difference $\big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big]$ for each $k$, we establish the following two properties. 
First, combining Lemma~\ref{lem:Qk-error} and the definition~\eqref{defn:V-Q} that $V_h^{k-1}(s_h^k) = \max_a Q^{k-1}_h(s^k_h, a)$, one can easily see that  
\begin{align}
	V_h^{k-1}(s_h^k) \ge Q^{k-1}_h(s^k_h, \pi^{\star}(s^k_h, h)) \ge Q^{\star}_h(s^k_h, \pi^{\star}(s^k_h, h)) = V^{\star}_h(s^k_h).
\end{align}
In addition, by definition $\pi_k(s_h^k, h) \defn a^k_h$, one can therefore decompose the difference $V_h^{k-1}(s_h^k) - V_h^{\pi_k}(s_h^k)$ as 
\begin{align}
\notag &V_h^{k-1}(s_h^k) - V_h^{\pi_k}(s_h^k) = Q^{k-1}_h(s^k_h, a^k_h) - Q^{\pi_k}_h(s^k_h, a^k_h) \\
%
\notag &= Q^{k-1}_h(s^k_h, a^k_h) - Q_h^{\star}(s^k_h, a^k_h) + Q_h^{\star}(s^k_h, a^k_h) - Q^{\pi_k}_h(s^k_h, a^k_h) \\
%
\notag &= Q^{k-1}_h(s^k_h, a^k_h) - Q_h^{\star}(s^k_h, a^k_h) + P_{h, s^k_h, a^k_h}(V^{\star}_{h+1} - V^{\pi_k}_{h+1}) \\
%
&= Q^{k-1}_h(s^k_h, a^k_h) - Q_h^{\star}(s^k_h, a^k_h) + \big(P_{h, s^k_h, a^k_h} - P^k_h\big)(V^{\star}_{h+1} - V^{\pi_k}_{h+1}) + V^{\star}_{h+1}(s^k_{h+1}) - V^{\pi_k}_{h+1}(s^k_{h+1}),
\end{align}
where the third line invokes Bellman equation $Q^{\pi}(s, a) = r(s, a) + P_{h, s, a}V^{\pi}$.
Combining these two properties leads to
\begin{align*}
&\sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big] \le \sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{k-1}(s_1^k) - V_1^{\pi_k}(s_1^k)\big] \\
&= \sum_{k \in \mathcal{I}_{1}^K}^K \big[V_2^{\star}(s_2^k) - V_2^{\pi_k}(s_2^k)\big] + \sum_{k \in \mathcal{I}_{1}^K} \big[Q^{k-1}_1(s^k_1, a^k_1) - Q_1^{\star}(s^k_1, a^k_1) + (P_{1, s^k_1, a^k_1} - P^k_1)(V^{\star}_{2} - V^{\pi_k}_{2})\big] \\
&\le \sum_{k \in \mathcal{I}_{2}^K}^K \big[V_2^{\star}(s_2^k) - V_2^{\pi_k}(s_2^k)\big] + \sum_{k \in \mathcal{I}_{1}^K} \big[Q^{k-1}_1(s^k_1, a^k_1) - Q_1^{\star}(s^k_1, a^k_1) + (P_{1, s^k_1, a^k_1} - P^k_1)(V^{\star}_{2} - V^{\pi_k}_{2})\big],
\end{align*}
where the last line comes from the observation that $\mathcal{I}_{h}^K \subset \mathcal{I}_{h+1}^K$ (cf.~\eqref{eq:defn-Ihk}).
Applying the above relation recursively yields that with probability at least $1-\delta$, the following inequality satisfies 
\begin{align*}
\sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big] &\le \sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} \big[Q^{k-1}_h(s^k_h, a^k_h) - Q_h^{\star}(s^k_h, a^k_h) 
+ (P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1})\big] \\
%
&\le \sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} b_h^{k-1}(s^k_h, a^k_h) + (P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1})\big]\\
%
&= \underbrace{\sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} b_h^{k-1}(s^k_h, a^k_h)}_{\Delta_1} + 
\underbrace{\sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} (P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1})\big]}_{\Delta_2},
\end{align*}
where the second inequality invokes Lemma~\ref{lem:Qk-error}. 
Now it is sufficient to bound $\Delta_1, \Delta_2$ respectively.
\begin{itemize}
\item Let us proceed with controlling term $\Delta_{2}$.
We first make the useful observation that $\{(P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1})\}$ forms a martingale difference sequence
as $\pi^k_j$ is determined by $Q_j^{k-1}(s_j^k, a)$, 
and the sequence satisfies $|(P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1})| \le H$.
It allows us to apply Azuma-Hoeffding inequality~\citep{azuma1967weighted}, which ensures with probability at least $1-\delta$, the following inequality satisfies 
\begin{align}
\label{eqn:delta2}
\notag \Delta_2 = \sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} (P_{h, s^k_h, a^k_h} - P^k_h)(V^{\star}_{h+1} - V^{\pi_k}_{h+1}) 
&\le H\sqrt{\sum_{h = 1}^H\left|\mathcal{I}_{h}^K\right|\log (\frac{2}{\delta})}\\
%
&\le \sqrt{H^3 K \log(\frac{2}{\delta})}.
\end{align}


\item In terms of term $\Delta_{1}$.
To start, by Cauchy-Schwarz inequality, one has 
\begin{align}
\Delta_1 = \sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} \beta \sqrt{\varphi_h(s^k_h, a^k_h)^{\top}\big(\Lambda_h^{k-1}\big)^{-1}\varphi_h(s^k_h, a^k_h)} 
\le \beta \sqrt{KH} \sqrt{\sum_{h = 1}^H\sum_{k \in \mathcal{I}_{h}^K} \varphi_h(s^k_h, a^k_h)^{\top}\big(\Lambda_h^{k-1}\big)^{-1}\varphi_h(s^k_h, a^k_h)}.
\end{align}
To further control the right hand side,  we recall the following result from \citep{abbasi2011improved}.
\begin{lemma} [\citep{abbasi2011improved}]
\label{lem:sum-normalized} 
\ytw{add statement}
\begin{equation}
\sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_{h}^i, a_{h}^i)^{\top}\big(\Lambda_h^{i-1}\big)^{-1}\varphi_h(s_{h}^i, a_{h}^i) 
\le 
2\log \left(\frac{\mathrm{det}\left(\Lambda_h^{k}\right)}{\mathrm{det}\left(\Lambda_h^{0}\right)}\right) \le 2d\log\left(\frac{k}{d}+1\right).
\end{equation}
\end{lemma}
Taken collectively, we are ensured that 
\begin{align}
\label{eqn:delta1}
	\Delta_1 \leq \beta\sqrt{KH} \cdot \sqrt{2Hd \log K} = H\beta\sqrt{2dK\log K}.
\end{align}
\end{itemize}
Putting everything together gives 
\begin{align}
% \label{eqn:piazzolla}
	 \sum_{k \in \mathcal{I}_{1}^K} \big[V_1^{\star}(s_1^k) - V_1^{\pi_k}(s_1^k)\big]
	 \le H\beta\sqrt{2dK\log K} + \sqrt{H^3K \log (\frac{2}{\delta})} 
%
	\le C\sqrt{d^2H^6K\log^2 \frac{K}{\delta}},
\end{align}
where the last inequality uses $\beta \defn c_{\beta} \sqrt{dH^4\log \frac{K}{\delta}}$.

The claimed inequality~\eqref{eq:regret-bound-main} therefore holds true by combining \eqref{eqn:piazzolla} with \eqref{eqn:buenos-aires} and \eqref{eq:number-leafs}.




%
% \yxc{mention where this lemma comes from.}

% Lemma~\ref{lem:Qk-error} and \ref{lem:number-nodes} are established through analyzing $\theta_h^k - \theta_h^{\star}$ by induction method in the following.


\subsection{Proof of Lemma~\ref{lem:Qk-error}}
\label{sec:pf-lem-qk}

Let
\begin{align*}
\overline{\pi}_k(s, h) \defn \min_a\left\{a \in \mathcal{A}_{h}^k(s) : b_h^k(s, a) < \min_{a \in \mathcal{A}_{h}^k(s)} b_h^k(s, a) + \zeta_k\right\}
\end{align*}
where
\begin{align*}
\mathcal{A}_{h}^k(s) \defn \left\{a : \varphi(s, a)^{\top}\theta_h^k > \max_{a:b_h^k(s, a) < \tau_k} \varphi(s, a)^{\top}\theta_h^k - 2\tau_k\right\}\qquad\text{with }\tau_k = \tau + \zeta_k.
\end{align*}
Then
\begin{align}
\theta_h^k = \big(\Lambda_h^{k}\big)^{-1} \sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\big[r_h(s_h^i, a_h^i) + \varphi_{h+1}(s_{h+1}^i, \overline{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k}\big].
\end{align}
First recalling that $\theta_h^k$ is updated via rule~\eqref{eqn:update-theta}, we are therefore enabled to write out the following decomposition 
\begin{align}
\label{eqn:decomposition}
\theta_h^k - \theta_h^{\widehat{\pi}_k} &= \big(\Lambda_h^{k}\big)^{-1} \Big\{\sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\big[r_h(s_h^i, a_h^i) + \varphi_{h+1}(s_{h+1}^i, \overline{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k}\big] - \Lambda_h^{k}\theta_h^{\widehat{\pi}_k}\Big\} \nonumber\\
&= \big(\Lambda_h^{k}\big)^{-1} \Big\{\sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\big[\varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k} - P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k}\big] - \lambda\theta_h^{\widehat{\pi}_k}\Big\}.
\end{align}
Here, 
%for
%\begin{align*}
%\omega_1 &\defn \min_a\left|\max_a Q_h^{\widehat{\pi}_k}(s, a) - 4\tau_k - Q_h^{\widehat{\pi}_k}(s, a)\right|, \\
%\omega_2 &\defn \min_a\left|\max_{a:b_h^k(s, a) < \tau_k} \varphi(s, a)^{\top}\theta_h^k - 2\tau_k - \varphi(s, a)^{\top}\theta_h^k\right|, \\
%\omega_3 &\defn \min_a\left|\min_{a \in \mathcal{A}_{h}^k(s)} b_h^k(s, a) + \zeta_k - b_h^k(s, a)\right|
%\end{align*}
%and
%\[
%\Delta_h^{k}(s) \defn \min\left\{\omega_1, \omega_2, \omega_2\right\},
%\]
we let
\begin{align*}
\widehat{\pi}_k(s, h) \defn \left\{
\begin{array}{ll}
\overline{\pi}_k(s, h), & \text{if } Q_h^{\widehat{\pi}_k}(s, \overline{\pi}_k(s, h)) > \max_a Q_h^{\widehat{\pi}_k}(s, a) - 4\tau_k; \\
\arg\max_a Q_h^{\widehat{\pi}_k}(s, a), & \text{otherwise, }
\end{array}
\right. 
\end{align*}
which implies with probability at least $1 - \delta$
\begin{align*}
\widehat{\pi}_k(s_{h+1}^i, h+1) = \overline{\pi}_k(s_{h+1}^i, h+1),\qquad\text{for }i \in \mathcal{I}_{h}^k,
\end{align*}
and
\begin{align*}
\left|\varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k} - V_{h+1}^{\widehat{\pi}_k}(s_{h+1}^i)\right| \le b_{h+1}^k(s_{h+1}^i, a_{h+1}^i),\qquad\text{for }i \in \mathcal{I}_{h}^k.
\end{align*}
In addition, the second equality holds by the definition of $\Lambda_h^{k}$ in equality~\eqref{eqn:def-Lambda-hk} and noticing 
\begin{align*}
\Lambda_h^{k}\theta_h^{\widehat{\pi}_k} = \sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\varphi_h(s_h^i, a_h^i)^{\top}\theta_h^{\widehat{\pi}_k} + \lambda \theta_h^{\widehat{\pi}_k} 
&= \sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)Q_h^{\widehat{\pi}_k}(s_h^i, a_h^i) + \lambda \theta_h^{\widehat{\pi}_k} \\
&= \sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\big[r_h(s_h^i, a_h^i) + P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k}\big] + \lambda \theta_h^{\widehat{\pi}_k},
\end{align*}
where the second and third equalities invoke the linear realizable assumption of $Q_h^{\widehat{\pi}_k}$ with $Q_{h+1}^{\widehat{\pi}_k} \ge Q_{h+1}^{\star} - \tau$ and the Bellman equation respectively. 
As a result, to control the difference $\theta_h^k - \theta_h^{\widehat{\pi}_k}$, it is sufficient to bound 
$\varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k} - P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k}$. 
We first consider the following decomposition 
\begin{align*}
\varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^k - P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k} &= \varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k} - V_{h+1}^{\widehat{\pi}_k}(s_{h+1}^i) \\
&\qquad+ V_{h+1}^{\widehat{\pi}_k}(s_{h+1}^i) - P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k}
\end{align*}
and for notational simplicity, we define 
\begin{subequations}
\begin{align}
\varepsilon_h^k &\defn \left[\varphi_h(s_h^i, a_h^i)^{\top}\theta_h^k - Q_h^{\widehat{\pi}_k}(s_h^i, a_h^i)\right]_{i \in \mathcal{I}_{h}^k}, \\
\delta_h^k &\defn \left[\varphi_{h+1}(s_{h+1}^i, \widehat{\pi}_k(s_{h+1}^i, h+1))^{\top}\theta_{h+1}^{k} - V_{h+1}^{\widehat{\pi}_k}(s_{h+1}^i)\right]_{i \in \mathcal{I}_{h}^k}, \\
\xi_h^k &\defn \left[V_{h+1}^{\widehat{\pi}_k}(s_{h+1}^i) - P_{h, s_h^i, a_h^i}V_{h+1}^{\widehat{\pi}_k}\right]_{i \in \mathcal{I}_{h}^k}, \\
\Phi_h^k &\defn \left[\varphi_h(s_h^i, a_h^i)\right]_{i \in \mathcal{I}_{h}^k}.
\end{align}
\end{subequations}
Putting things together, $\theta_h^k - \theta_h^{\widehat{\pi}_k}$ can be written as 
\begin{align} 
\label{eqn:decomposition-new}
\theta_h^k - \theta_h^{\widehat{\pi}_k} = 
\big(\Lambda_h^{k}\big)^{-1} \Big\{\Phi_h^k \big(\delta_{h}^k + \xi_h^k\big) - \lambda\theta_h^{\widehat{\pi}_k}\Big\}.
\end{align}



We are ready to bound $Q_h^k(s, a) - Q_h^{\widehat{\pi}_k}(s, a)$ as required in Lemma~\ref{lem:Qk-error}.
Invoking inequality~\eqref{eqn:decomposition-new} directly yields 
\begin{align} 
&\big|\varphi_h(s, a)^{\top}\theta_h^k - Q_{h}^{\widehat{\pi}_k}(s, a)\big| =
\big|\varphi_h(s, a)^{\top}(\theta_h^k - \theta_h^{\widehat{\pi}_k})\big|\nonumber\\
%
&= \left|\varphi_h(s, a)^{\top}\big(\Lambda_h^{k}\big)^{-1}\Big\{\Phi_h^k\big(\delta_{h}^k+\xi_h^k\big) - \lambda\theta_h^{\widehat{\pi}_k}\Big\}\right| \nonumber\\
%
&\le \|\big(\Lambda_h^{k}\big)^{-1/2}\varphi_h(s, a)\|_2 \left(\|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\delta_{h}^k\|_2 + \|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\xi_h^k\|_2 + \lambda\|\big(\Lambda_h^{k}\big)^{-1/2}\theta_h^{\widehat{\pi}_k}\|_2\right), \nonumber
\end{align}
where the last inequality uses the Cauchy-Schwarz inequality and triangle inequality.
Now by definition 
\begin{align}
	\Lambda_h^{k} &= \sum_{i \in \mathcal{I}_{h}^k} \varphi_h(s_h^i, a_h^i)\varphi_h(s_h^i, a_h^i)^{\top} + \lambda I = \Phi_h^k (\Phi_h^k)^\top  + \lambda I,
\end{align}
it is easily seen that $\|\big(\Lambda_h^{k}\big)^{-1/2}\| \le \lambda^{-1/2}$ and $\|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\| \le 1$. 
Consequently, it is guaranteed that 
\begin{align}
\label{eqn:eps-decomposition}
\big|\varphi_h(s, a)^{\top}\theta_h^k - Q_{h}^{\star}(s, a)\big|
	&\le \big(\|\delta_{h}^k\|_2 + \|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\xi_h^k\|_2 + \sqrt{\lambda}\left\|\theta_h^{\star}\right\|_2\big) \cdot \|\big(\Lambda_h^{k}\big)^{-1/2}\varphi_h(s, a)\|_2.
\end{align}


\paragraph{Proof of inequality~\eqref{eq:Qk-error}:} We are now ready to establish---which shall be done by induction method---that 
\begin{align} \label{eq:error-Qk}
\big|\varphi_h(s, a)^{\top}\theta_h^k - Q_{h}^{\widehat{\pi}_k}(s, a)\big| \le b_h^{k}(s, a).
\end{align}
It is easily seen that \eqref{eq:error-Qk} directly implies the claimed inequality~\eqref{eq:Qk-error}, combining with the definition of $Q_h^{k}(s, a)$ as in~\eqref{eqn:update-Q}.


To begin with, let us establish a key inequality that shall be crucial for proving our target inequality~\eqref{eq:error-Qk}---that is with probability at least $1-\delta,$ for all $1\leq j \leq H$ and $1\leq k \leq K$, 
\begin{align}
\label{eqn:xi-bound}
	\left\|\big(\Lambda_j^{k}\big)^{-1/2}\Phi_j^k\xi_j^k\right\|_2
	\leq \sqrt{H^2(d\log K +2d\log\frac{HK}{\delta})}.
\end{align}
Towards this, let us define $X_i \defn V(s_{j+1}^i) - P_{j, s_j^i, a_j^i}V$, where 
\begin{align*}
V(s) = \varphi_{j+1}(s, \pi(s))^{\top}\widehat{\theta}
\end{align*}
with $\pi = \widehat{\pi}$.
Consider the following virtual sample sequence:
for each $(s_j^i, a_j^i)$, we generate $N$ independent transitions $s_{j+1}^{i, n} \sim \mathbb{P}(\cdot\mymid s_j^i, a_j^i)$, $n = 1, 2, \ldots, N$.
Then
\begin{align}
\Big\|\big(\Lambda_j^{k}\big)^{-1/2} \sum_{i \in \mathcal{I}_{j}^k}\frac{1}{N} \big[\sum_{n = 1}^N V(s_{j+1}^{i, n}) - P_{j, s_j^i, a_j^i}V\big]\Big\|_2
\end{align}
Let $\mathcal{N}_{\epsilon}(\theta)$ and $\mathcal{N}_{\epsilon}(\Lambda)$ denote $\epsilon$-nets for $\theta$ and $\Lambda^{-1}$, respectively.
\begin{align}
\Big\|\big(\Lambda_j^{k}\big)^{-1/2} \sum_{i \in \mathcal{I}_{j}^k} \big[V(s_{j+1}^{i}) - \frac{1}{N} \sum_{n = 1}^N V(s_{j+1}^{i, n})\big]\Big\|_2
\end{align}
It is easily seen that $X_{i}$ forms a martingale sequence with regard to randomness of $\{(s_\ell^m, a_\ell^m)\}_{\ell\leq j, m\leq i}.$
Therefore we are ensured that 
\begin{align}
\left\|\big(\Lambda_j^{k}\big)^{-1/2}\Phi_j^k\xi_j^k\right\|_2 = 
\Big\|\big(\Lambda_j^{k}\big)^{-1/2} \sum_{i \in \mathcal{I}_{j}^k}\varphi_j^iX_i\Big\|_2 
&\le 
\sqrt{H^2\log\left(\frac{\mathrm{det}\left(\Lambda_j^{k}\right)}{\mathrm{det}\left(\Lambda_j^{0}\right)\delta^2}\right)}  \nonumber\\
&\le \sqrt{H^2(d\log K +2\log\frac{1}{\delta})} 
\label{eqn:xi-bound-pre}
\end{align}
holds with probability at least $1-\delta$.
Here, the first inequality comes from the fact that $|X_i| \le H$ combined with Lemma~\ref{lem:normalized}; the last inequality holds since $\|\varphi_h(s, a)\|_2 \le 1$ and 
 $\log (\frac{\mathrm{det}\left(\Lambda_j^{k}\right)}{\mathrm{det}\left(\Lambda_j^{0}\right)}) \le d\log K$
 (as a result of Lemma~\ref{lem:sum-normalized}).
 Taking an union bound of \eqref{eqn:xi-bound-pre} over $j=1,\ldots, H$ and $k=1,\ldots, K$ yields the required relation~\eqref{eqn:xi-bound}. 


\begin{lemma}[Concentration of self-normalized processes \citet{abbasi2011improved}] \label{lem:normalized}
Assume $\left\{X_t\right\}_{t = 1}^{\infty}$ is a martingale corresponding to the filtration $\left\{\mathcal{F}_t\right\}_{t = 0}^{\infty}$ with
\begin{align}
\mathbb{E}\left[X_t \mymid \mathcal{F}_{t-1}\right] = 0, \qquad\text{and}\qquad \mathbb{E}\left[e^{\lambda X_t} \mymid \mathcal{F}_{t-1}\right] \le e^{\frac{\lambda^2\sigma^2}{2}},~\forall~\lambda \in \mathbb{R}.
\end{align}
In addition, suppose that $\varphi_t \in \mathbb{R}^d$ is a random vector over $\mathcal{F}_{t-1}$, and $\Lambda_t = \Lambda_0 + \sum_{i = 1}^t \varphi_i\varphi_i^{\top}$ for some positive definite matrix $\Lambda_0 \in \mathbb{R}^{d\times d}$.
Then, with probability at least $1-\delta$, one has
\begin{align}
\Big\|\left(\Lambda_t \right)^{-1/2} \sum_{i = 1}^t \varphi_iX_i\Big\|_2^2 \le \sigma^2\log\left(\frac{\mathrm{det}(\Lambda_t)}{\mathrm{det}(\Lambda_0)\delta^2}\right)
\end{align}
holds for all $t \ge 0$.
\end{lemma}

Now we move on to demonstrate inequality~\eqref{eq:error-Qk} by induction method. First notice that when $h = H+1$, inequality~\eqref{eq:error-Qk} holds true trivially.
Let us assume that the claim holds for $h+1, \ldots, H+1$.
Then it is sufficient to consider the case at $h$-th step through bounding the terms in \eqref{eqn:eps-decomposition} separately.

\begin{itemize}


\item {\bf The term $\|\delta_{j}^k\|_2$.}
By induction assumption, inequality~\eqref{eq:error-Qk} holds for $h+1,\ldots, H+1$ which guarantees that
for $h \leq j \leq H$, one has 
\begin{align*}
V_{j+1}^{\star}(s_{j+1}^i) = Q_{j+1}^\star(s_{j+1}^i, \pi^\star(s_{j+1}^i)) &\leq \varphi_h(s_{j+1}^i, \pi^\star(s_{j+1}^i))^{\top}\theta_{j+1}^{i-1} + b_{j+1}^{i-1}(s_{j+1}^i, \pi^\star(s_{j+1}^i)) \\
&\leq
\varphi_h(s_{j+1}^i, a_{j+1}^i)^{\top}\theta_{j+1}^{i-1} + b_{j+1}^{i-1}(s_{j+1}^i, a_{j+1}^i),
\end{align*}
where $(\mathrm{i})$ uses the fact that $a_{j}^i$ maximizes $Q_j^{i-1}(s_j^i, a) = \varphi_h(s_{j}^i, a)^{\top} \theta_j^{i-1} + b_j^{i-1}(s_{j}^i, a)$. At the same time, we have 
\begin{align*}
\qquad Q_{j+1}^{\star}(s_{j+1}^i, a_{j+1}^i) &\ge \varphi_h(s_{j+1}^i, a_{j+1}^i)^{\top}\theta_{j+1}^{i-1} - b_{j+1}^{i-1}(s_{j+1}^i, a_{j+1}^i).
\end{align*}

It further gives
\begin{align*}
0 \le V_{j+1}^{\star}(s_{j+1}^i) - Q_{j+1}^{\star}(s_{j+1}^i, a_{j+1}^i) \le 2b_{j+1}^{i-1}(s_{j+1}^i, a_{j+1}^i),
\qquad
i \in \mathcal{I}_{j}^k.
\end{align*}
Then by the choice of $i \in \mathcal{I}_{j}^k$, \ytw{check the index; old notes have $i \in \mathcal{I}_{j-1}^k$.} one has $b_j^{i-1}(s_{j}^i, a_{j}^i) \leq \tau$, 
and the sub-optimality gap assumption, we have
\[
V_{j+1}^{\star}(s_{j+1}^i) - Q_{j+1}^{\star}(s_{j+1}^i, a_{j+1}^i) = 0,\qquad\text{for all }i \in \mathcal{I}_{j}^k,
\]
and hence
\begin{align}
\|\delta_{j}^k\|_2 = 0. \label{eqn:delta-bound}
\end{align}

\begin{comment}
Then combined with the suboptimality gap assumption, the above relation yields
\begin{align}
\|\delta_{j-1}^k\|_2^2 &\le \frac{1}{64d}\sum_{i \in \mathcal{I}_{j-1}^k} 4b_j^{i-1}(s_{j}^i, a_{j}^i)^2 \nonumber\\
&\le \frac{1}{64d}\sum_{i \in \mathcal{I}_{j}^k} 4c^2dH^4\varphi_j(s_{j}^i, a_{j}^i)^{\top}\big(\Lambda_j^{i-1}\big)^{-1}\varphi_j(s_{j}^i, a_{j}^i)\log \frac{K}{\delta} \nonumber\\
&\le \frac{c^2}{16}dH^4\log \frac{K}{\delta}, \label{eqn:delta-bound}
\end{align}
where the last line comes from Lemma~\ref{lem:sum-normalized}.
Notice that we needs the suboptimality gap assumption to restrict the error spread of $\delta_{j}^k$ and then to avoid the exponential blow-up.
If $\tau < \Delta_{\mathcal{M}}$, $\delta_{j}^k$ becomes zero. \gen{Then we expect for some relatively large $\tau$, this goal can be achieved.}
\end{comment}

\item {\bf The term $\|\varepsilon_{h+1}^k\|_2$.}
Recall that inequality~\eqref{eqn:decomposition-new} allows us to write $\varepsilon_h^k$ in the following manner 
\begin{align*}
\varepsilon_h^k = \left(\Phi_h^k\right)^{\top}\left(\theta_h^k - \theta_h^{\star}\right) = \left(\Phi_h^k\right)^{\top}\big(\Lambda_h^{k}\big)^{-1}\Big\{\Phi_h^k\big(\left[\varepsilon_{h+1}^k\right]_{i \in \mathcal{I}_{h}^k}+\delta_{h}^k+\xi_h^k\big) - \lambda\theta_h^{\star}\Big\}.
\end{align*}
Combining with basic properties $\|(\Phi_h^k)^{\top}\big(\Lambda_h^{k}\big)^{-1/2}\| \le 1$, $\|\big(\Lambda_h^{k}\big)^{-1/2}\| \le \lambda^{-1/2}$, and $\mathcal{I}_{h}^K \subset \mathcal{I}_{h+1}^K$, 
leads to
\begin{align}
\|\varepsilon_h^k\|_2 &= \left\|\left(\Phi_h^k\right)^{\top}\big(\Lambda_h^{k}\big)^{-1}\Big\{\Phi_h^k\big(\left[\varepsilon_{h+1}^k\right]_{i \in \mathcal{I}_{h}^k}+\delta_{h}^k+\xi_h^k\big) - \lambda\theta_h^{\star}\Big\}\right\|_2 \nonumber\\
&\le \left\|\varepsilon_{h+1}^k\right\|_2+\left\|\delta_{h}^k\right\|_2+\|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\xi_h^k\|_2 + \sqrt{\lambda}\left\|\theta_h^{\star}\right\|_2.
\end{align}
Applying the above inequality recursively yields 
\begin{align}
\|\varepsilon_h^k\|_2 &\le \left\|\varepsilon_{H+1}^k\right\|_2 + \sum_{h \le j \le H} \Big[\|\delta_{j}^k\|_2+\|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_j^k\xi_j^k\|_2 + \sqrt{\lambda}\|\theta_j^{\star}\|_2 \Big] \nonumber\\
&\le 2\sqrt{dH^4\log \frac{KH}{\delta}}. \label{eqn:eps-bound}
\end{align}
where the last inequality holds by putting together $\varepsilon_{H+1}^k = 0$, inequalities~\eqref{eqn:xi-bound} and \eqref{eqn:delta-bound} and the assumption that $\|\theta_j^{\star}\|_2 \leq H\sqrt{d}$. 

\end{itemize}

Combining inequalities~\eqref{eqn:xi-bound}, \eqref{eqn:delta-bound}, \eqref{eqn:eps-bound} with relation~\eqref{eqn:eps-decomposition}, we arrive at 
\begin{align}
	\big|\varphi_h(s, a)^{\top}\theta_h^k - Q_{h}^{\star}(s, a)\big|
	% &\le \big(\|\varepsilon_{h+1}^k\|_2 + \|\delta_{h}^k\|_2 + \|\big(\Lambda_h^{k}\big)^{-1/2}\Phi_h^k\xi_h^k\|_2 + \sqrt{\lambda}\left\|\theta_h^{\star}\right\|_2\big) \cdot \|\big(\Lambda_h^{k}\big)^{-1/2}\varphi_h(s, a)\|_2\\
	%
	\notag &\le 
	(2\sqrt{dH^4\log \frac{KH}{\delta}}
	+ \sqrt{H^2(d\log K +2\log\frac{HK}{\delta})} + H\sqrt{d})\|\big(\Lambda_h^{k}\big)^{-1/2}\varphi_h(s, a)\|_2\\
	%
	&\le c_{\beta} \sqrt{dH^4\log \frac{KH}{\delta}}\|\big(\Lambda_h^{k}\big)^{-1/2}\varphi_h(s, a)\|_2 = b_h^k(s,a)
\end{align}
which completes the induction step of \eqref{eq:error-Qk}, thus the proof of Lemma~\ref{lem:Qk-error}.




\subsection{Proof of Lemma~\ref{lem:number-nodes}}
\label{sec:invierno-porteno}

As a direct consequence of Lemma~\ref{lem:sum-normalized}, one has 
\begin{align*}
\sum_{k \in \mathcal{I}_{h+1}^K} b_{h+1}^{k-1}(s_{h+1}^k, a_{h+1}^k)^2 
&\le \sum_{k \in \mathcal{I}_{h+1}^K} c^2dH^4\varphi_{h+1}(s_{h+1}^k, a_{h+1}^k)^{\top}\big(\Lambda_{h+1}^{k-1}\big)^{-1}\varphi_{h+1}(s_{h+1}^k, a_{h+1}^k)\log \frac{K}{\delta} \\
%
&\le c^2d^2H^4\log^2 \frac{K}{\delta}.
\end{align*}
It implies that there are at most $\frac{c^2d^2H^4\log \frac{K}{\delta}}{\tau^2}$ samples in $\mathcal{I}_{h+1}^K$ with $b_{h+1}^{k-1}(s_{h+1}^k, a_{h+1}^k) > \tau$, which means 
\begin{align*}
\left|\mathcal{I}_{h+1}^K \setminus \mathcal{I}_{h}^K\right| \le \frac{c^2d^2H^4\log^2 \frac{K}{\delta}}{\tau^2}.
\end{align*}
We complete the proof of Lemma~\ref{lem:number-nodes}.


